Forward and Inverse models in HCI:Physical simulation and deep learning for inferring 3D finger pose

We outline the role of forward and inverse modelling approaches in the design of human--computer interaction systems. Causal, forward models tend to be easier to specify and simulate, but HCI requires solutions of the inverse problem. We infer finger 3D position $(x,y,z)$ and pose (pitch and yaw) on a mobile device using capacitive sensors which can sense the finger up to 5cm above the screen. We use machine learning to develop data-driven models to infer position, pose and sensor readings, based on training data from: 1. data generated by robots, 2. data from electrostatic simulators 3. human-generated data. Machine learned emulation is used to accelerate the electrostatic simulation performance by a factor of millions. We combine a Conditional Variational Autoencoder with domain expertise/models experimentally collected data. We compare forward and inverse model approaches to direct inference of finger pose. The combination gives the most accurate reported results on inferring 3D position and pose with a capacitive sensor on a mobile device.

==> gp.tex <==
\graphicspath{{../../simon/matlab/150414/}{GPchapter/}}


\clearpage
\section{GPs for z, pitch and yaw}

To generate the plots in this report, run:
\begin{verbatim}
	simon/matlab/forrod/gp_script_final.m
\end{verbatim}

\subsection{Data}
\begin{verbatim}
cylsim_updated/dataset10cm1, randdataset10cm1,  randdataset10cm2,  randdataset10cm3,
\end{verbatim}
This dataset contains a mix of two types of data. One group is 400 points generated by the simulator at a systematic range of positions and angles. The simulated finger had a radius of 7mm and length of 10cm. These points ranged such that the lowest point of the finger was positioned at  $x=0.02:0.035$, $y=0.04:0.06$, and $z=0.3cm:3.5cm$ at pitch angles of $0,30,60,90\degr$ and yaw angles of $-60,-45,0,45,60 \degr$.
A further $581$ points were generated randomly in the same $x,y,z$ range and at pitch angles from 0 to 90  and yaw angles from $-90\degr$ to $90\degr$. 

We normalise the sensor values for each training and testing example so that the maximum value of the whole set is 1. 75\% of the data (681 points) were used for training and 25\% (227 points) for testing.

\section{Results on raw data}
\subsection{Predicting z}
Using the \texttt{gpml} toolbox (\url{http://www.gaussianprocess.org/gpml/code/matlab/doc/}), an RBF covariance function (\texttt{covSEard}) with automatic relevance detection and using marginal likelihood maximisation to optimise the hyperparameters, We used a \ac{GP} to predict the $z$ value. The data were normalised such that the mininum sensor value was 0 and the maximum 1 (across the whole dataset).\\

 Performance is given as \ac{RMSE} (in mm) from partitions of the data into a training test (75\%) and a test set (25\%). An example of the predictions (with standard deviations) can be seen in Figure~\ref{fig:zcomp_direct}.\\


\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{zbox_direct.pdf}		
	%\caption{Performance of $z$ prediction.}
	\label{fig:zbox}
	\includegraphics[width=0.47\linewidth]{zcomp_direct.pdf}	}	
	\caption{\label{fig:zcomp_direct}Example of $z$ predictions with all sensor information. Grey lines show predictive standard deviation.}
\end{figure}

\subsection{Predicting yaw}

Using the same setup as in the previous example, we attempt to predict the yaw value (Figure~\ref{fig:layout_top}).  The results can be seen in Figure~\ref{fig:yawbox_direct}. The second boxplot in Figure~\ref{fig:yawbox_direct} is a baseline constructed by predicting $0\degr$ for each test point.\\

\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{yawbox_direct.pdf}	
	\label{fig:yawbox_direct}	
	%\caption{\label{fig:yawbox_direct}Performance of yaw prediction.}
	\includegraphics[width=0.47\linewidth]{yawcomp_direct.pdf}		
	\caption{\label{fig:yawcomp_direct}Example of yaw predictions with all sensor information. Grey lines show predictive standard deviation.}}
\end{figure}


\subsection{Predicting pitch}

Using the same setup as in the previous example, we attempt to predict the yaw value (Figure~\ref{fig:layout_top}).  The results can be seen in Figure~\ref{fig:pitchbox_direct}. The second boxplot in Figure~\ref{fig:pitchbox_direct} is a baseline constructed by predicting $0\degr$ for each test point.\\


\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{pitchbox_direct.pdf}
	\label{fig:pitchbox_direct}		
	%\caption{Performance of pitch prediction.}
	\includegraphics[width=0.47\linewidth]{pitchcomp_direct.pdf}}	
	\caption{\label{fig:pitchcomp_direct}Example of pitch predictions with all sensor information. Grey lines show predictive standard deviation.}
\end{figure}


\clearpage

\section{Centring data via a $5 \times 5$ pixel filter}
\subsection{Processing}
\begin{figure}[tbh]
	\includegraphics[width=0.6\linewidth]{capvals.pdf}		
	\centering\caption{\label{fig:capvals}Visualisation of cap sensor values, showing the possible window regions.}
\end{figure}

To reduce the training set required, we experimented with cropping the array for each input to include only those sensors that were active (i.e. those around the end of the virtual finger). Figure~\ref{fig:capvals} gives an example. Each square is a sensor sensor, and the three blocks show three different sizes of regions that could be extracted. The regions are always centred on the highest sensor value, and the assumption is that this is below the lowest point of the finger.

\clearpage
\subsection{Predicting z}
Using the \texttt{gpml} toolbox (\url{http://www.gaussianprocess.org/gpml/code/matlab/doc/}), an RBF covariance function (\texttt{covSEard}) with automatic relevance detection and using marginal likelihood maximisation to optimise the hyperparameters, We used a \ac{GP} to predict the $z$ value. The data were normalised such that the mininum sensor value was 0 and the maximum 1 (across the whole dataset).\\

 Performance is given as \ac{RMSE} (in mm) from partitions of the data into a training test (75\%) and a test set (25\%). An example of the predictions (with standard deviations) can be seen in Figure~\ref{fig:zcomp_filter2}.\\


\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{zbox_filter2.pdf}		
	%\caption{Performance of $z$ prediction.}
	\label{fig:zbox_filter2}
	\includegraphics[width=0.47\linewidth]{zcomp_filter2.pdf}	}	
	\caption{\label{fig:zcomp_filter2}Example of $z$ predictions with a  $5 \times 5$ pixel filter. Grey lines show predictive standard deviation.}
\end{figure}

\subsection{Predicting yaw}

Using the same setup as in the previous example, we attempt to predict the yaw value (Figure~\ref{fig:layout_top}).  The results can be seen in Figure~\ref{fig:yawbox_filter2}. The second boxplot in Figure~\ref{fig:yawbox_filter2} is a baseline constructed by predicting $0\degr$ for each test point.\\


\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{yawbox_filter2.pdf}		
	%\caption{Performance of yaw prediction.}
	\label{fig:yawbox_filter2}
	\includegraphics[width=0.47\linewidth]{yawcomp_filter2.pdf}	}	
	\caption{\label{fig:yawcomp_filter2}Example of yaw predictions with a  $5 \times 5$ pixel filter. Grey lines show predictive standard deviation.}
\end{figure}


\subsection{Predicting pitch}

Using the same setup as in the previous example, we attempt to predict the yaw value (Figure~\ref{fig:layout_top}).  The results can be seen in Figure~\ref{fig:pitchbox_filter2}. The second boxplot in Figure~\ref{fig:pitchbox_filter2} is a baseline constructed by predicting $0\degr$ for each test point.\\


\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{pitchbox_filter2.pdf}		
	%\caption{Performance of pitch prediction.}
	\label{fig:pitchbox_filter2}
	\includegraphics[width=0.47\linewidth]{pitchcomp_filter2.pdf}}		
	\caption{\label{fig:pitchcomp_filter2}Example of pitch predictions with a  $5 \times 5$ pixel filter. Grey lines show predictive standard deviation.}
\end{figure}


\clearpage

\section{Centring data via a $3 \times 3$ pixel filter}
\subsection{Predicting z}
\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{zbox_filter1.pdf}		
	%\caption{Performance of $z$ prediction.}
	\label{fig:zbox_filter1}
	\includegraphics[width=0.47\linewidth]{zcomp_filter1.pdf}	}	
	\caption{\label{fig:zcomp_filter1}Example of $z$ predictions with a a $3 \times 3$ pixel filter filter. Grey lines show predictive standard deviation.}
\end{figure}

\subsection{Predicting yaw}

Using the same setup as in the previous example, we attempt to predict the yaw value (Figure~\ref{fig:layout_top}).  The results can be seen in Figure~\ref{fig:yawbox_filter1}. The second boxplot in Figure~\ref{fig:yawbox_filter1} is a baseline constructed by predicting $0\degr$ for each test point.\\


\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{yawbox_filter1.pdf}		
	%\caption{Performance of yaw prediction.}
	\label{fig:yawbox_filter1}
	\includegraphics[width=0.47\linewidth]{yawcomp_filter1.pdf}	}	
	\caption{\label{fig:yawcomp_filter1}Example of yaw predictions with a a $3 \times 3$ pixel filter filter. Grey lines show predictive standard deviation.}
\end{figure}

\subsection{Predicting pitch}

Using the same setup as in the previous example, we attempt to predict the yaw value (Figure~\ref{fig:layout_top}).  The results can be seen in Figure~\ref{fig:pitchbox_filter1}. The second boxplot in Figure~\ref{fig:pitchbox_filter1} is a baseline constructed by predicting $0\degr$ for each test point.\\


\begin{figure}[tbh]
	\centering{\includegraphics[width=0.47\linewidth]{pitchbox_filter1.pdf}		
	%\caption{Performance of pitch prediction.}
	\label{fig:pitchbox_filter1}
	\includegraphics[width=0.47\linewidth]{pitchcomp_filter1.pdf}}		
	\caption{\label{fig:pitchcomp_filter1}Example of pitch predictions with a a $3 \times 3$ pixel filter filter. Grey lines show predictive standard deviation.}
\end{figure}


\clearpage











\comment{

To generate the plots in this report, run..:
\begin{verbatim}
	simon/matlab/150414/gp_script.m
\end{verbatim}

\subsection{Data}
\begin{verbatim}
simulator_stuff/dataset5
\end{verbatim}
This dataset contains 100 points generated by the simulator. Each simulated finger position used a pitch angle of $60\degr$ from the vertical. The lowest point of the finger was positioned at random $(x,y,z)$ co-ordinates and random yaw values at $\pm89\degr$ from a line parallel to the $y$-axis of the screen.

\subsection{Processing}
\begin{figure}[tbh]
	\includegraphics[width=0.7\linewidth]{capvals.pdf}		
	\centering\caption{\label{fig:capvals}Visualisation of cap sensor values, showing the possible window regions.}
\end{figure}

To reduce the training set required, I experimented with cropping the array for each input to include only those sensors that were active (i.e. those around the end of the virtual finger). Figure~\ref{fig:capvals} gives an example. Each square is a sensor sensor, and the three blocks show three different sizes of regions that could be extracted. The regions are always centered on the highest sensor value, and the assumption is that this is below the lowest point of the finger.

\subsection{Predicting z}
Using the \texttt{gpml} toolbox (\url{http://www.gaussianprocess.org/gpml/code/matlab/doc/}), an RBF covariance function (\texttt{covSEard}) with automatic relevance detection and using marginal likelihood maximisation to optimise the hyperparameters, I used a \ac{GP} to predict the $z$ value. The data were normalised such that the mininum sensor value was 0 and the maximum 1 (across the whole dataset).\\

Figure~\ref{fig:zbox} shows the performance for the smallest box size (no measurable improvement was observed) by increasing the box width. Performance is given as \ac{RMSE} (in mm) and 50 different partitions of the data into a training test (75\%) and a test set (25\%) were used. An example of the predictions (with standard deviations) can be seen in Figure~\ref{fig:zexample}.\\


\begin{figure}[tbh]
	\includegraphics[width=0.7\linewidth]{zbox_filter1.pdf}		
	\centering\caption{\label{fig:zbox}Performance of $z$ prediction for a $3\times 3$ box. Boxes shown in Figure~\ref{fig:capvals}}
\end{figure}
\begin{figure}[tbh]
	\includegraphics[width=0.7\linewidth]{zexample_filter1.pdf}		
	\centering\caption{\label{fig:zexample}Example of $z$ predictions. Grey lines show predictive standard deviation.}
\end{figure}

To demonstrate how little information is needed to provide a good prediction of $z$, Figure~\ref{fig:zbox_high} shows the performance when only the value of the most active sensor is used Performance is close to that of the $3\times 3$ grid. An example of predictions is given in Figure~\ref{fig:zexample_high}.\\

\begin{figure}[tbh]
	\includegraphics[width=0.7\linewidth]{zbox_high_filter1.pdf}		
	\centering\caption{\label{fig:zbox_high}Performance of $z$ prediction for a $3\times 3$ box. Boxes shown in Figure~\ref{fig:capvals}}
\end{figure}
\begin{figure}[tbh]
	\includegraphics[width=0.7\linewidth]{zexample_high_filter1.pdf}		
	\centering\caption{\label{fig:zexample_high}Example of $z$ predictions. Grey lines show predictive standard deviation.}
\end{figure}

\section{$3 \times 3$ pixel window}

\clearpage

\subsection{Predicting yaw}

Using the same setup as in the previous example, we attempt to predict the yaw value (Figure~\ref{fig:layout_top}). The only difference between this and the previous experiments is that we normalise the sensor values \emph{for each training and testing example} so that the maximum value is 1. The results for a $3\times 3$ grid can be seen in Figure~\ref{fig:yawbox}. The second boxplot in Figure~\ref{fig:yawbox} is a baseline constructed by predicting $0\degr$ for each test point.\\

\begin{figure}[tbh]
	\includegraphics[width=0.7\linewidth]{yawbox_filter1.pdf}		
	\centering\caption{\label{fig:yawbox}Performance of yaw prediction for a $3\times 3$ box. Boxes shown in Figure~\ref{fig:capvals}}
\end{figure}
% \begin{figure}[tbh]
% 	\includegraphics[width=0.7\linewidth]{yawexample_filter1.pdf}		
% 	\centering\caption{\label{fig:yawexample}Example of yaw predictions. Grey lines show predictive standard deviation.}
% \end{figure}

To try and improve performance, we can increase the grid to $5\times 5$. The performance can be seen in Figure~\ref{fig:yawbox_filter2}. There is a marked improvement in performance.

\begin{figure}[tbh]
	\includegraphics[width=0.7\linewidth]{yawbox_filter2.pdf}		
	\centering\caption{\label{fig:yawbox_filter2}Performance of yaw prediction for a $5\times 5$ box. Boxes shown in Figure~\ref{fig:capvals}}
\end{figure}
% \begin{figure}[tbh]
% 	\includegraphics[width=0.7\linewidth]{yawexample_filter2.pdf}		
% 	\centering\caption{\label{fig:yawexample_filter2}Example of yaw predictions. Grey lines show predictive standard deviation.}
% \end{figure}

\section{GP experiments with new simulator data}
This section describes experiments with Pellikka's simulation.


\subsection{Predictions over whole space}

\subsubsection{$z$ prediction}

\subsubsection{Yaw prediction}

\subsubsection{Pitch prediction}


\subsection{`Re-centred' results}

}

==> particlefilter.tex <==
\clearpage
\subsection{Particle filter approach}
\begin{figure}[htb!]
    \centering
    \includegraphics[width=\linewidth]{FwdInvPF.pdf}
    \caption{Particle filter components, showing the role of the forward and inverse models.}
    \label{fig:my_label}
\end{figure}
We implemented a particle filter to perform \textit{stateful} tracking; i.e. to track the inferred finger pose over time. The particle filter (or sequential Monte Carlo filter) is a probabilistic predictor-corrector, which maintains an estimate of distribution over possible finger poses $P\left( {\bf y_t} \right), \quad {\bf y_t} = \left[x_t,y_t,z_t,\theta_t,\phi_t\right]$ as a set of discrete samples. It updates this distribution by weighting samples according to how close their expected sensor state would be to true observations of the sensor ${\bf X}$. Heavily weighted samples are propagated forward in time, and low weight samples are discarded. Internal dynamics which model the potential evolution of inferred finger poses allow the filter to predict likely future states when observations are noisy or incomplete. As shown in Figure~\ref{fig:my_label}, we use both our forward model which predicts $\bf{\hat{X}}$ given ${\bf y}$ (to predict the sensor states we would expect from an estimated internal state) \textbf{and} our inverse model which predicts ${\bf \hat{y} }$ from $\bf X$ in the filter. In each prediction step, we have a set of samples of possible states for $\bf y$. We apply a weighting step first based on the forward model, then a second weighting step based on the inverse model, before performing the importance sampling step. This allows our model to automatically and transparently cope when one of the two models is underdetermined. In testing with trajectory tracking, this particle filter outperforms our best inverse model, as well as having much more stable and smooth dynamics. We tested both the forward model and the particle filter on a 315 frames sequence. The particle filter approach was comparable on $(x,y,z)$, less subject to sudden jitter, and performed with around 30\% reduction of RMSE on the pitch estimation. It also provides full probabilistic confidence estimates rather than single point observations. We observed that the particle filter approach decreased the variability of the predictions, and was more robust to application without explicit calibration than the regression approach. We show the results as an example of PF inference for a human movement with the real sensor in Figure~\ref{fig:dynamicTouchTraj}.
\begin{figure}[htb!]
\includegraphics[width=0.95\linewidth]{pf_series_typing_3D.pdf}
\includegraphics[width=\linewidth]{pf_series_typing_sensor.pdf}
\centerline{\includegraphics[width=\linewidth]{pf_series_typing}}
\caption{A finger moving from one position to another. The sensor readings are shown at samples during the trajectory. Below that we see the particle filter inference about the states during the trajectory.}
\label{fig:dynamicTouchTraj}
\end{figure}
